SnatchML: Hijacking ML models without Training Access

Model hijacking can cause significant accountability and security risks since the owner of a hijacked model can be framed for having their model offer illegal or unethical services. Prior works consider model hijacking as a training time attack, whereby an adversary requires full access to the ML model training. In this paper, we consider a stronger threat model for an inference-time hijacking attack, where the adversary has no access to the training phase of the victim model. Our intuition is that ML models, which are typically over-parameterized, might have the capacity to (unintentionally) learn more than the intended task they are trained for. We propose SnatchML, a new training-free model hijacking attack, that leverages the extra capacity learnt by the victim model to infer different tasks that can be semantically related or unrelated to the original one. Our results on models deployed on AWS Sagemaker showed that SnatchML can deliver high accuracy on hijacking tasks. Interestingly, while all previous approaches are limited by the number of classes in the benign task, SnatchML can hijack models for tasks that contain more classes than the original. We explore different methods to mitigate this risk; We propose meta-unlearning, which is designed to help the model unlearn a potentially malicious task while training for the original task. We also provide insights on over-parametrization as a possible inherent factor that facilitates model hijacking, and accordingly, we propose a compression-based countermeasure to counteract this attack. We believe this work offers a previously overlooked perspective on model hijacking attacks, presenting a stronger threat model and higher applicability in real-world contexts.

==> sec/02_intuition.tex <==

\begin{figure*}[htp]
  \centering
  \includegraphics[width=0.85\linewidth]{general_figures/corr_er_fr.pdf}
  \caption{Correlation distribution between output feature maps from pretraine Emotion Recognition and Face Recognition.}
  \label{fig:corr3}
\end{figure*}

\section{Intuition and Preliminary Analysis}\label{sec:intuition}

 We posit that the models might learn more than they should in the training process, including learning other tasks. Our intuition is that ML models, perhaps due to over-parametrization, have a by-design capacity that exceeds the minimum necessary capacity to learn the task they are trained for. While it has been shown in the literature that models can overfit and memorise data making them vulnerable to certain attacks such as Membership \cite{reza} and property inference \cite{pia} attacks, the risk that ML models (unintentionally) generalize to other tasks is yet to be explored/exploited.
In this section, we provide a preliminary analysis to gain insights in the plausibility of this hypothesis. Given a model $f^{(i)}(.)$ trained on a data distribution $(X,Y) \sim \mathcal{D}$, using a loss function $\mathcal{L}_i$, relevant to a Task $\mathcal{T}_i$. Let $f^{(j)}(.)$ be a model with the same architecture as $f^{(i)}(.)$, but is trained  on a data distribution $(X’,Y’) \sim \mathcal{D}’$, using a loss function $\mathcal{L}_j$, relevant to a Task $\mathcal{T}_j \neq \mathcal{T}_i$. We ask whether
features learnt by $f^{(i)}(.)$ are correlated with those learnt by $f^{(j)}(.)$? 
We train two ResNet-9 and two Mobilenet architectures each for both Emotion Recognition and Face Recognition. We then check the correlation coefficient distribution between the same layers’ features maps that correspond to the 2 tasks.  
The correlation coefficient between two variables $X$ and $Y$, denoted as $r$, is defined as:
\begin{equation}
    r = \frac{\sum_{i=1}^n (X_i - \overline{X})(Y_i - \overline{Y})}{\sqrt{\sum_{i=1}^n (X_i - \overline{X})^2} \sqrt{\sum_{i=1}^n (Y_i - \overline{Y})^2}}
\end{equation}
where:
\begin{itemize}
    \item $n$ is the number of data points,
    \item $X_i$ and $Y_i$ are the individual values of the variables $X$ and $Y$,
    \item $\overline{X}$ and $\overline{Y}$ are the means of $X$ and $Y$ respectively.
\end{itemize}

% The value of $r$ ranges from -1 to 1, where:
% \begin{itemize}
%     \item $r = 1$ indicates a perfect positive linear relationship,
%     \item $r = -1$ indicates a perfect negative linear relationship,
%     \item $r = 0$ indicates no linear relationship between the variables.
% \end{itemize}

Figure \ref{fig:corr3} shows the features correlation distribution for Layer 5 and layer 11 for ResNet-9, and Layer 2 and Layer 4 for Mobilenet. Intrestingly, Figure \ref{fig:corr3} shows a positive correlation suggesting a potential overlap between what the model learns for tasks that share semantic clues. In other words, this preliminary observation supports the idea that models trained on an original task are capable of extracting features relevant to other tasks. 

% \ihsen{A good idea maybe we would represent the latent low dimensional space by t-SNE of a model $f_i()$ on a task Ti and $f_j()$ on task Ti; how close the features distribution of $D_i$ when projected by $f_i()$ and by $f_j()$. Can $f_j()$ project the input in the latent space close enough to the projection of $f_i()$ ?}
% \textcolor{blue}{We briefly explain the intuition, and show the preliminary analysis about features correlation (briefly) }
% \begin{itemize}
%     \item \textcolor{blue}{@Mahmoud: the objective of the preliminary analysis is to show that there is (positive) correlation of learnt features between tasks. Nothing more. So instead of using the previous results which are layer wise, we can take any features layer and check the correlation distribution across a subset of data samples --  }
    
% \end{itemize}




==> sec/08_attack_analysis.tex <==
% \section{Attack Analysis}

% \subsection{Impact of task complexity ratio}

% \subsection{Impact of limited output classes}



==> sec/4-2_AR.tex <==
%\section{Action Recognition models are Biometric Identifiers}

\subsection{Context}
Over the past few years, intelligent surveillance cameras have been deployed in streets, stadiums, airports and other public places for security reasons. One of the tasks that these systems are expected to perform is to recognize human actions to flag potential incidents such as violent situations.



While in some countries, such as China, laws allow the government to use facial recognition and identity identification techniques, in other countries, like France, this technique is strictly prohibited due to privacy concerns when facial expression recognition FER is allowed. 
%Debates regarding regulating AI-powered systems are now taking place in the European Union (EU), and the proposed risk-based approach from the European Commission has been particularly prominent in this regard. These debates focus on issues like privacy concerns, potential for discrimination, and the requirement for accountability. 
%This discussion becomes more pertinent in light of the approaching 2024 Olympic Games in Paris, where France's stringent laws prohibiting face recognition and person identification techniques intersect with the delicate balance between addressing security needs and preserving public freedom. The controversy surrounding the French government's planned utilization of AI-based surveillance cameras for the 2024 Paris Olympic Games accentuates the complexities of this balance.
It is, therefore, essential to ensure that FER models cannot be used for facial identification.

\subsection{Setup}
\textbf{Dataset: KTH Action dataset }
The KTH Action dataset \cite{schuldt2004recognizing}, known as KTH, is a widely used dataset featuring six actions: walk, jog, run, box, hand-wave, and hand clap. Each action is executed by 25 different individuals, and the setting is systematically changed for each actor to capture performance nuances. The settings include outdoor, outdoor with scale variation, outdoor with different clothes, and indoor. These variations assess the algorithms' capability to recognize actions regardless of background, actor appearance, and actor scale.


\textcolor{blue}{\textit{Ihsen--} \hl{Rmodels etc etc --} }

% \subsection{AR as biometric identifiers}

% \textcolor{blue}{\textit{Ihsen--} \hl{Results for AR here--} }

% \subsection{AR Systems recognize gender}


==> sec/Previous_reviews.tex <==
\pagebreak
\clearpage
% \newpage

% \begin{center}
%    \underline{ \textbf{Reviews from NDSS2025 Submission}}
% \end{center}

% \noindent \textbf{Review \#1136C}


% \noindent \textbf{Paper Summary}
% The paper proposes a hijacking attack named SnatchML, which enables model hijacking during inference without requiring access to the model’s training process. Additionally, the paper introduces two defensive methods to counter SnatchML: model compression and meta-unlearning.

% \noindent \textbf{Strengths:}
% \begin{itemize}
%     \item The attack eliminates the need for access to training, making SnatchML a potentially significant threat.
%     \item The number of classes in the hijacking task can exceed those of the original task.
% \end{itemize}

% \noindent \textbf{Weaknesses:}
% \begin{itemize}
%     \item The distinctiveness of the attack should be clarified in certain cases.
%     \item Some findings lack detailed analysis.
%     \item Several key baselines are missing from the evaluation of defenses.
% \end{itemize}


% \noindent \textbf{Detailed Comments for Authors}
% This paper proposes SnatchML, a model hijacking attack that requires only inference access to the victim model. The core of SnatchML resembles contrastive learning, making predictions for a new task based on the distance between the embeddings (logits or intermediate representations) of an attacker-controlled labeled data point and another input during inference. Based on observations from these attacks, the paper introduces model compression and meta-unlearning as defenses to mitigate such hijacking attempts.

% \begin{itemize}
%     \item The definition of BEK could be improved. The current definition does not clearly show the relationship between $h(\cdot)$, $x$, and $\zeta_h(\cdot)$.
    
%     \item What distinguishes user re-identification from membership inference? The paper describes the latter as identifying users whose data were used to train the ER model, which closely resembles a membership inference attack. What makes this hijacking attack stand out as a new threat, if that's the case?
    
%     \item The paper considers an upper bound on attack performance in several experiments. Why was the unconstrained version of the previous attack [40] chosen as the upper bound? The reasoning behind this selection could be clarified. Additionally, why not directly compare with [40] in these experiments?
    
%     \item The attack's performance on ECG diagnosis is better than in other cases. What is the reason behind this?
    
%     \item In the model compression defense, why not simply remove neurons with small weights during computation? Pruning-based methods could also be useful here, and these should serve as baselines to justify the need for a new defense.
    
%     \item Meta-unlearning bears some similarities to non-transferable learning \cite{wang2021non}. Comparing these two approaches would further solidify the paper's contribution.
    
%     \item Some typos should be fixed:
%     \begin{itemize}
%         \item Olivetti Faces $\to$ Olivetti Faces, Page 3
%         \item [40] in the References should be fixed.
%     \end{itemize}
% \end{itemize}

% \noindent \textbf{Concrete Steps for Improvement}
% \begin{itemize}
%     \item Include additional baselines in the evaluation of defenses.
    
%     \item Provide thorough reasoning and motivations for the experimental setup in the attack evaluation.
    
%     \item Offer a more detailed analysis of the experimental results.
    
%     \item Refine the BEK definition and elaborate on the uniqueness of the attack.
% \end{itemize}


% \noindent \textbf{Review \#1136B}
% \textbf{Paper summary}: The paper's main motivation is to explore the possibility of hijacking machine learning models (called model hijacking) at inference time, even when the attacker has no access to the training process (black-box scenario), and for this, the paper aims to demonstrate that models can be repurposed for potentially malicious tasks without requiring any modification to the model itself or access to its training data. SnatchML is introduced - an approach that leverages the unintentional learning capabilities of benign models to repurpose them for potentially malicious tasks at inference time, even when the hijacking task is unrelated to the original task. The paper aims to challenge the conventional understanding of model security and raise important questions about the potential risks associated with the widespread deployment of machine learning models. \\
% \textbf{Strengths}:
% \begin{itemize}
%     \item The goal behind SnatchML is definitely exciting, which is to leverage the unintentional learning capabilities of benign models to repurpose them for potentially malicious tasks at inference time, even when the hijacking task is unrelated to the original task. Given the widespread deployment of machine learning models, this is an important problem that surfaces significant risks associated with ML training.
%     \item The paper provides a comprehensive evaluation of SnatchML across various domains and tasks, showcasing its effectiveness and generalizability.
% \end{itemize}
% \textbf{Weaknesses}:

% \textit{Technical Limitations}:
% \begin{itemize}
%     \item A more in-depth comparison between SnatchML and existing model hijacking attacks (KNN) to highlight unique contributions, because Section 3 seems similar to KNN. Additionally, in Sec XIII the conceptual similarities between SnatchML and transfer learning, particularly Adversarial Reprogramming (AR) makes it confusing what is the key distinction. Except that AR requires optimization and/or additional training of the NN, which isn't necessarily a bad thing.
%     \item Although the SnathML's goal is to demonstrate the attack even without training access, the underperforming tasks can benefit from some explanation even if the performance isn't always superior.
% \end{itemize}

% \textit{Writing Clarity}:
% \begin{itemize}
%     \item Section III: SnatchML: General Approach, Sec. X: Why Do ML Models Learn More Than They Should?, and the algo 1 presentation needs to be written with more clarity and can have a few illustrative examples or diagrams. As they are, the details are making reading very hard to follow.
% \end{itemize}

% \textit{Theory}:
% \begin{itemize}
%     \item The theoretical descriptions in sec. X for model hijacking discusses the universality of random DNNs and their ability to perform unrelated tasks by referring to Johnson-Lindenstrauss Lemma [26] and Giryes et al. [18], however, just stating that these provide insights is not sufficient. It would be helpful if the authors could strengthen the theoretical framework by expanding these connections and offering further insights into the observed patterns or phenomena. Or conduct additional experiments to support their claim.
%     \item Section XI (Countermeasures), where 2 defense approaches are proposed: model compression and meta-unlearning requires more in-depth analysis of the strengths and weaknesses of each defense, discusses their practical implication.
% \end{itemize}

% \textit{Minor Weaknesses}:
% \begin{itemize}
%     \item A more detailed explanation of the experimental setup and methodology.
% \end{itemize}

% \textbf{Detailed comments for authors}: Overall, the paper presents a problem that if addressed, can make a valuable contribution to the field of machine learning security by highlighting a novel and concerning threat model for model hijacking attacks. The proposed SnatchML framework and the comprehensive evaluation provide compelling evidence of the feasibility and potential impact of such attacks. However, the paper could be further strengthened by addressing the identified weaknesses, including improving clarity, correcting grammatical errors, strengthening theoretical explanations, and expanding the discussion of defense mechanisms. I think the paper warrants further investigation.

% \textbf{Concrete steps for improvement}:
% \begin{itemize}
%     \item Carefully review and revise the paper to enhance clarity and presentation, particularly in sections with complex technical details or explanations.
%     \item Thoroughly proofread the paper to identify and correct grammatical errors and typos.
%     \item Provide more rigorous analysis and formalization to support the theoretical explanations for the observed phenomena, particularly the ability to hijack models for unrelated tasks.
%     \item Review and refine arguments and explanations to ensure clarity, and logical coherence, and avoid confusion.
%     \item Provide a more comprehensive discussion of the limitations and potential trade-offs associated with the proposed defense mechanisms.
% \end{itemize}

% \noindent \textbf{Review \#1136C}
% \textbf{Paper summary}: Proposed in the paper a hijacking attack named SnatchML, which enables model hijacking during inference without requiring access to the model’s training process. Additionally, the paper introduces two defensive methods to counter SnatchML: model compression and meta-unlearning. \\
% \textbf{Strengths}:
% \begin{itemize}
%     \item The attack eliminates the need for access to training, making SnatchML a potentially significant threat.
%     \item The number of classes in the hijacking task can exceed those of the original task.
% \end{itemize}
% \textbf{Weaknesses}:
% \begin{itemize}
%     \item Overlap with KNN.
%     \item Missing illustrations to support Section XI.
%     \item Performance metrics need further explanation.
% \end{itemize}

% \textbf{Detailed comments for authors}: The authors present an interesting attack on the use of machine learning models and attempt to highlight its potential impact through a series of experimental evaluations. While the problem itself is compelling and presents new avenues for research, the presentation of the paper leaves much to be desired. Several sections (Section III in particular) require clarification, and the similarities between SnatchML and KNN should be explicitly addressed to distinguish the contribution. Further explanation is required to justify the proposed defenses.




% \noindent \textbf{Review \#1136A}
% \textbf{Paper summary}: This article proposes a method to redirect pre-trained models without training, and names it testing time model hijacking attacks. The paper also discusses potential defenses. \\
% \textbf{Strengths}:
% \begin{itemize}
%     \item Timely follow novel model hijacking attack
% \end{itemize}
% \textbf{Weaknesses}:
% \begin{itemize}
%     \item The method lacks novelty.
%     \item Performance is not enough to support motivation.
%     \item Most of the findings have been previously reported.
%     \item The generalizability of the conclusions is questionable.
%     \item The writing is confusing.
% \end{itemize}
% \textbf{Detailed comments for authors}: 

% First of all, I would like to thank the authors for their work. However, I spent quite a long time reading this article, fail to grasp the core contribution of the article, and have a lot of confusion. I hope the authors can clarify them.

% Basically, I think the method in this article can be summarized as: a feature space is created by the pre-trained model (which may be an unrelated task). Then, in this feature space, the KNN algorithm is used (each cluster has only one data point) to perform classification. From my side, I think SnatchML may be just another name of transfer learning. My detailed question is: 
% \begin{enumerate}
%     \item What is the difference between the labeling method in Section 3 and KNN?
%     \item What is the difference between this method and transfer learning [frozen model + classifier (this classifier KNN)]?
%     \item And what is the difference between it and pre-trained model (note that many pre-trained models are also unrelated tasks) + KNN?
% \end{enumerate}
% The performance does not seem competitive. It is obviously weaker than other method / using other transfer learning classifier. For example, in Figure 9, the accuracy of MNIST is about 80\% with MobileNet. It is almost free to train an MNIST classifier with an accuracy of more than 95\%. What do the authors think about this problem?

% Considering the KNN (please allow me to temporarily call it KNN) is only considering one data point (the advantage the authors claim), the results will potentially be not robust. The results depend a lot on the selected sample in each class. What do the authors think about this issue?

% The findings and root cause exploration of this article appear to be outdated and be previously reported. There are many existing articles on root cause analysis of transfer learning. For example, [1] claims that ``Many transfer learning methods assume that the source tasks and the target task be related, even though many tasks are not related in reality. However, when two tasks are unrelated, the knowledge extracted from a source task may not help, and even hurt, the performance of a target task.''. [1]'s finding even covers/refutes this paper's finding.

% The article was written in a hurry, which makes it difficult to understand. For example, UB in Figure 15 cites [43], while the main text cites [40]. The author of [40] does not seem to exist?

% In summary, I think most of the work in this paper has been done before, and some previous work is even more comprehensive than this one. The authors need to address the problem of novelty, the performance and motivation, the robustness concern, writing issues. \\


% \begin{center}
%     \textbf{** Edits to the manuscript to address the reviewers' feedback **}
% \end{center}


% \noindent\textbf{[Common Concerns]}\\
% 1. \textbf{Novelty} - [Reviewer A-B]: We edited the manuscript's framing and writing to present the novelty of this paper in a clearer manner. Specifically, we highlighted:
% \begin{itemize}
%     \item[$(a)$] \textbf{The novel threat-model compared to existing hijacking attacks} While SnatchML is effective in the traditional 'framing the model owner' scenario, it is equally applicable in a different context where the model owner deliberately misuses a benign model for covert malicious purposes. In this setting, the model owner does not alter the model or the input, making their actions difficult to detect. For instance, consider a situation where a CCTV camera is employed by authorities or a company for a legitimate purpose, such as emotion recognition, using a model from a trusted vendor. With SnatchML, the same model can be repurposed on the same input stream for malicious activities, such as tracking specific minorities, without any modifications to the input data or the model itself.

%     \item[(b)] \textbf{Approach novelty compared to core hijacking-attacks:} (i) In contrast with the main hijacking approaches in the literature, SnatchML does not require access to the victim model's training. (ii) Unlike all previous hijacking attacks, we propose the first approach that is not constrained by the number of classes in the victim model.

%     \item[$(c)$] \textbf{Novelty over Adversarial-Reprogramming:} In Section \ref{sec:related} , we discuss the main advantages of our approach over AR: (i) AR requires editing the input. It therefore cannot be used in scenario point[$(1)$]. (ii) Like other hijacking attacks, AR is limited by the number of classes in the victim model. SnatchML isn’t. (iii) AR requires a white-box access to the model to use the gradient for the optimisation. SnatchML can work in a black-box setting.
% \end{itemize}

% 2. \textbf{Transfer-learning/KNN} - [Reviewer A-B]
% We edited the paper to emphasize the differences in the objectives and similarities in the mechanics of the inference part of our approach. In fact, SnatchML can be framed as a zero-shot transfer learning method, where the pre-trained model remains entirely frozen and is repurposed for a new, potentially unrelated task in a black-box setting. The inference process operates like a k-nearest neighbor (KNN) approach with $k=1$, using features extracted from a pre-trained model on a distribution different from the one being inferred upon.

% 3. \textbf{Writing clarity/typos:[Reviewer B-C]} We improved the writing in this version and corrected the typos for a better readability.



% \noindent\textbf{[Reviewer B]}\\
% 1. \textbf{Comparison with KNN-Hijacking:} We are not aware of existing KNN-based hijacking approaches. %We kindly ask the reviewer to point us to the reference to compare with.

% 2. \textbf{Cases with low success:} We provided more detailed discussion of the limitation of our approach in Section \ref{sec:disc}. 
% %Because of its zero-shot aspect, the performance of SnatchML can be significantly affected by the distribution of the hijacking task (inter-class/intra-class variance). For instance, in scenarios like ethnicity classification, different ethnic groups might have significant intra-class variance. We will provide a more thorough analysis of the cases where our approach is not performing well, would we have a chance to revise the paper.


% 3. \textbf{Experiments to back theory:} We provide additional results on different datasets (MNIST, Cifar100, ImageNet, CK+ Emotions, CK+ Identities, Olivetti, Celebrity, Synthetic) with different models on experimental settings that corroborate the theoretical insights such as randomly initialized models to back the random projection hypothesis.  Results are shown in the Appendix in Tables \ref{tab:resnet-18-imagenet}, \ref{tab:mobilenet-imagenet}, \ref{tab:Resnet_50_cifar10}, \ref{tab:mobilenet_cifar10} and \ref{tab:2d_cnn_random}.

% \noindent\textbf{[Reviewer C]}\\
% We clarified the potential confusion on several points including  \textbf{Re-identification vs. Membership Inference}, the choice of the \textbf{Upper-bound} We select the unconstrained version of [43] based on our assumption of an extreme poisoning-for-hijacking attack where the adversary has full control over the model and training dataset. We have results compared with [43], which is weaker than the upper bound.

% \noindent\textbf{Model Compression/Pruning:} We tested both structured and unstructured saliency-based pruning methods yielded similar results to our proposed compression technique. This is because conventional saliency measures neuron/weight importance with respect to the original task, not the hijacking task. %Advanced pruning methods (e.g., where saliency is guided by explainability with respect to both original and hijacking tasks) are needed for better performance.

% \noindent\textbf{Comparing with Non-Transferable Learning:} The NTL approach is designed to restrict the learning to specific domains, and prevent learning on target domain \textbf{within the same task}. We discuss the similarity with our meta-unlearning defense in Section \ref{sec:meta-unlearn}.

% %Our goal is different: we want to prevent the attacker from reusing knowledge from the victim model to perform a new task, whereas non-transferable learning only targets the accessibility of the parameters. We will clarify this difference in the revised version.




==> sec/x2_peliminary.tex <==

\section{Preliminary analysis}
As shown in Figure \ref{fig:correlations} (a), a model with the same architecture, trained separately for facial emotion recognition and facial recognition, reveals a remarkable correlation pattern: a high correlation in the first layers which decreases gradually. This pattern is reproduced in figure \ref{fig:correlations} (b), showing the correlation between action recognition and person identification. These observations fuel our hypothesis that machine learning models, despite their conventional training for specific tasks, unintentionally accumulate features conducive to unintended applications, notably in biometric identification. Using this correlation-based analysis, we delve deeper into the broader privacy implications, highlighting the potential risks associated with deploying machine learning models in security-sensitive areas and making the case for a more nuanced understanding of privacy in the training and application of these models.




\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/mobilenet_correlation.pdf}
        \caption{Emotion Recognition vs. Face Recognition in Inverted Residual Blocks of \texttt{MobileNet}}
        \label{fig:correlation_a}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/resnet_correlation.pdf}
        \caption{Emotion Recognition vs. Face Recognition in Residual Blocks of \texttt{ResNet-9}}
        \label{fig:correlation_b}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/r3d_18average_correlation-1.pdf}
        \caption{Action Recognition vs. Person Identification in Residual Blocks of \texttt{r3d\_18}}
        \label{fig:correlation_c}
    \end{subfigure}
    \caption{Correlations between biometric recognition and EM/AR across Various Models}
    \label{fig:correlations_subfigures}
\end{figure*}


==> sec/x6_experiments.tex <==

\section{Experiments}
% \subsection{Creation of a new dataset}
% Datasets simultaneously providing labels for emotions and identities have been relatively rare, preventing extensive research and experimentation. The insufficiency of these dual-labeled datasets has been a limiting factor in the development and validation of models to recognize individuals' emotional states and their unique identities. Understanding the nuanced relationship between emotions and individual identity in facial expressions required a richer data set encompassing a broad range of emotional expressions across diverse identities.

% To fill this gap, we created a dataset that would serve as a valuable resource for researchers, allowing them to delve deeper into the intricacies of facial emotions analysis and potential identity privacy vulnerabilities. By providing a meticulously labeled dataset featuring known and unknown individuals expressing various emotions, we aimed to facilitate more robust and comprehensive studies and experiments in the field. 


\subsection{Datasets}

\textbf{CK+:}
The Extended Cohn-Kanade (CK+) dataset \cite{lucey2010extended}, a foundational dataset for facial expression analysis, contains 593 video clips from 123 individuals between the ages of 18 and 50. These videos capture transitions between neutral and focused peak expressions: anger, disgust, fear, happiness, sadness, and surprise. CK+ is widely recognized as a pivotal, extensively used database for facial expression classification methods.

\textbf{new-dataset:}
 We built a new dataset labeled for emotions and identities to carry out the attack on identity based on FER features. This dataset was created using MakeHuman \cite{bastioni2008ideas}, an open-source tool designed to simplify the creation of virtual humans using a Graphical User Interface. The generated dataset consists of 405 images, each of which is labeled for both emotions and identities. There are a total of 57 unique identities within the dataset, which are divided into two categories:



\begin{itemize}
      \item \textbf{Unknown Identities (10):} These 10 identities are only associated with the "neutral" emotional expression. This means that for each of these individuals, only one image is available in the dataset, and they are all depicted with a neutral facial expression.
    
      \item \textbf{Known Identities (47):}
     In contrast to the unknown identities, these 47 individuals are each associated with not only the "neutral" emotional expression but also with 6 distinct facial expressions, resulting in a total of 7 different emotional states per identity. This comprehensive labeling allows for a more detailed analysis of emotional expressions across various individuals.
     \textcolor{red}{we should maybe use another expression instead of known and unknown}
\end{itemize}

The labeling of emotions in the dataset is conducted according to the FER features, making it suitable for studies and experiments related to identity-based attacks using facial recognition technology. By providing images of known and unknown individuals expressing different emotions, this dataset becomes a valuable resource for research and experimentation in facial recognition and emotional analysis.

\textbf{Emotion and Identity Labeled Dataset of Famous Faces}

We meticulously created a dataset of 79 facial images featuring famous individuals in order to advance our experiments. This collection began with 13 neutral expressions gathered from Google. Using specialized tools, we generated 66 emotion-specific images from these neutrals. These images are labeled for seven emotions and associated with 13 unique individuals, serving dual roles in facial emotion recognition (FER) and identity classification (ID). This valuable resource can be utilized by researchers and practitioners in computer vision for further exploration and experimentation.


It was expertly annotated for seven distinct emotions (anger, disgust, fear, happiness, sadness, surprise, and neutral), as well as identity labels. The dataset encompasses 13 images displaying neutral expressions, 66 images conveying various emotions, and 13 unique identities. The dataset's dual purpose is to facilitate facial emotion recognition (FER) and identity classification (ID) tasks, making it an invaluable resource for researchers and practitioners in the field of computer vision.

\subsection{FER to Identification}
During the experiment, ResNet-9 \cite{he2016deep},  MobileNet \cite{howard2017mobilenets} and a 2D Convolutional Neural Network (2D-CNN) were used to perform the task of FER ( \(FER\)-model). The 2D-CNN, used in articles \cite{allaert2022comparative, poux2021dynamic}, consists of three convolutional layers, each followed by ReLU activation and max-pooling. The convolutional layers progressively extract hierarchical features from the input image. The classifier includes two fully connected layers, with the first layer reducing dimensionality through ReLU activation and the final layer produces class predictions.  The three models were trained with a learning rate of 0.001, using the Cross-Entropy loss function, for a total of 10 epochs for MobileNet and 2D-CNN, and 15 epochs for ResNet-9. The code was executed in Google Colab with a T4 GPU for accelerated training and computation. Our study focused on a subset of the Extended Cohn-Kanade (CK+) dataset, specifically selecting 975 images representing 98 distinct identities. In creating the subset, we followed the strategy outlined in the article \cite{allaert2022comparative}, which selects 10 frames per sequence to attempt to impose the same pace of expression activation. These images were derived from the final frames of video clips capturing diverse emotional expressions, including anger, disgust, fear, happiness, sadness, and surprise. We divided the dataset into training, validation, and test sets, with proportions of 70\%, 10\%, and 20\%, respectively. as mentioned in section \ref{subsec:Method}, the first step is to train the \(FER\)-model using only the emotion label \(Y\). In the evaluation phase, the classification accuracy served as the metric for assessing our model's performance. The three models used as \(FER\)-model have proven their effectiveness in recognizing facial emotions by giving results greater than 95\% as shown in Figure \ref{fig:accuracy}.
\par
After training the \(FER\)-model, we recovered the feature maps \(F\) extracted before the classification and we associate each feature map \(F\) with its identity \(ID\). In this way, we create a dataset of the form (\(F, ID\)) (We extracted emotion-related features from the \(FER\)-model at a specific layer, which we then saved together with their respective IDs). Then, using these emotion-based features, we trained an \(ID\)-model to perform face recognition. During our investigation, we tested both KNN and CNN as   \(ID\)-models. In the inference step, we used the \(FER\)-model to extract the pertinent emotion-related features for the test dataset. The identities of these test images were then predicted using the trained \(ID\)-model.
Starting from the observation that we made about the variation of the correlation across the different layers between a model designed for ER and a model designed for ID, we judged it good to take the features learned by FER-model at different layers to see the impact it will have on the precision of the ID-model.


\begin{figure}
     \centering
     \begin{subfigure}[b]{0.47\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{images/accuracy_mobilenet.pdf}
        \caption{ \texttt{MobileNet} on CK+.}
        \label{fig:sub_mobilenet}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.47\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{images/accuracy_resnet-2.pdf}
        \caption{ \texttt{ResNet-9} on CK+.}
        \label{fig:sub_resnet}
     \end{subfigure}
     \hfill
\caption{Performance Analysis: ID-Model Classification Accuracies in \texttt{MobileNet} and \texttt{ResNet-9} Across Various Layers on CK+ Test subdataset.}
\label{fig:accuracy}
\end{figure}


% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.95\linewidth]{images/mobilenet_submodels_acc.png}
%   \caption{acc per layers MobileNet}
%   \label{fig:sub_mobilenet}
% \end{figure}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.95\linewidth]{images/resnet_submodls_acc.png}
%   \caption{acc per layers ResNet-9}
%   \label{fig:sub_resnet}
% \end{figure}
While our experiment demonstrated the effectiveness of the \textit{FER}-model in performing the facial emotion recognition (FER) task, the transition to the \textit{ID}-model for user re-identification revealed an intriguing bias. The \textit{FER}-model, originally designed for facial emotion recognition, unsurprisingly exhibited exceptional performance due to its dedicated training on emotional labels. However, the real insight lies in the performance of the \textit{ID}-model, which was trained to identify individuals based on emotion-related features extracted from the \textit{FER}-model. The \textit{ID}-model achieved high classification accuracy in the initial layers of the ResNet-9 and MobileNet models when predicting identities from these emotion-based features. Subsequently, the classification accuracy dropped in the subsequent layers, consistent with our initial observation of correlations. While these results may appear significant, they unveil an intriguing bias between features learned for ER and used for facial recognition.

While the classification accuracy declined in the subsequent layers of the \textit{ID}-model, the utilization of the top-k metric unveiled an unsettling revelation. Despite the drop in accuracy, the top-k metric showcased that the true identity persisted within the k nearest samples. This is a significant finding that underscores a substantial privacy risk.

The persistence of the true identity within the top-k nearest samples, even amidst the accuracy decline, magnifies the privacy implications. This suggests that, despite a slight reduction in the model's ability to precisely identify an individual, it remains proficient at narrowing down the possible identities within a close proximity.

Figure \ref{fig:topk-k} underscores the significance of the top-k metric in highlighting the vulnerability of individuals' privacy. The results depicted in Subfigures \ref{fig:topkmobilnet} and \ref{fig:topkresnet} showcase the Top-5 classification accuracy for user re-identification based on features extracted from the 4th Residual Block of MobileNet and 4th Residual Block of ResNet-9, respectively, using the CK+ test subdataset. Notably, as k increases, the precision also elevates.

Despite both models exhibiting relatively low accuracy at Top-1, the top-k metric reveals an unsettling truth: even if the model fails to precisely identify the exact individual, it maintains the capability to include the true identity within the k nearest samples. This presents a significant threat to privacy, implying that while an individual's identity might not be precisely determined, it could be highly probable among a select few closest matches. Such a scenario potentially compromises their anonymity and privacy.

This observation accentuates the criticality of understanding the implications of increasing k in re-identification tasks. With an increase in k, the model's capacity to include the true identity within the top-k matches rises, intensifying the privacy risks associated with potential identification among the nearest samples. Responsible consideration and stringent measures are imperative to mitigate these privacy threats, ensuring the ethical use of models and safeguarding individuals' anonymity and privacy.

In reality, even greater precision than chance is significant and highlights the risks to privacy. The key observation here is that the performance of the \textit{ID}-model, although slightly lower than that of the \textit{FER}-model, remain remarkably accurate in identifying individuals on the basis of features initially intended for the recognition of emotions. This highlights the potential for unintentional data leakage from models like \textit{FER}-model, where emotion recognition and user identification intersect.

The existence of this bias is a stark reminder of the need for stricter safeguards and ethical considerations when processing data related to facial emotions. Even a seemingly modest drop in accuracy when transitioning from the \textit{FER} model to the \textit{ID} model reaffirms the privacy risks associated with deploying models in contexts for which they were not originally intended, highlighting the importance of responsible data management and responsible use of models. 

\section{experiment results}




\begin{table}[h]
  \centering
  \begin{tabular}{@{}lcccccc@{}}
    \toprule
    Model & Top-1 & Top-2 & Top-3 & Top-4 & Top-5 \\
    \midrule
    ID-KNN & 40.31\% & 59.57\% & 65.96\% & 65.96\% & 70.21\% \\
    \bottomrule
  \end{tabular}
  \caption{Top-k Accuracy Results for ID-KNN}
  \label{tab:accuracy_knn}
\end{table}

\begin{table}[h]
  \centering
  \resizebox{0.47\textwidth}{!}{%
    \begin{tabular}{@{}lcccccc@{}}
      \toprule
      Model & Test 1 & Test 2 & Test 3 & Test 4 & Test 5 & Average \\
      \midrule
      AR-model & 79.12 & 89.47 & 78.94 & 99.41 & 97.45 & 96.82 \\
      ID-KNN & 62.95 & 47.37 & 47.37 & 80.10 & 87.76 & 83.17 \\
      \bottomrule
    \end{tabular}
  }
  \caption{Test Accuracy Results obtained for Weizmann dataset.}
  \label{tab:accuracy}
\end{table}



%\begin{table}[h]
%  \centering
%  \begin{tabular}{@{}lcccccc@{}}
%    \toprule
%    Model & Top-1 & Top-2 & Top-3 & Top-4 & Top-5 \\
%    \midrule
%    ID-KNN & 16.76\% & 27.13\% & 35.77\% & 39.58\% & 47.15\% \\
%    \bottomrule
%  \end{tabular}
%  \caption{Accuracy of the top-k Results for ID-KNN on KTH action recognition dataset}
%  \label{tab:kth-top}
%\end{table}


%\begin{table}[h]
 % \centering
 % \begin{tabular}{@{}lcccccc@{}}
 %   \toprule
 %   Model & Top-1 & Top-2 & Top-3 & Top-4 & Top-5 \\
 %   \midrule
 %   ID-KNN & 37.76\% & 48.13\% & 54.77\% & 60.58\% & 65.15\% \\
 %   \bottomrule
 % \end{tabular}
 % \caption{Accuracy of the top-k Results for ID-KNN on KTH action recognition dataset}
 % \label{tab:kth-top}
\%end{table}

\begin{table}[h]
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    dataset & Test Accuracy (\%) \\
    \midrule
    Virtual-faces & 95.74 \\
    Feamous-real-faces & 100 \\
    \bottomrule
  \end{tabular}
  \caption{Test Accuracy Results for the attack}
  \label{tab:accuracy2}
\end{table}



%\begin{table}[h]
%  \centering
%  \resizebox{0.49\textwidth}{!}{%
%    \begin{tabular}{@{}lccc@{}}
%      \toprule
%      Noise & FER-model & ID-CNN & ID-KNN \\
%      \midrule
%      0.01 & 89.27 / 97.21 / 92.35 & 92.86 /91.84 / 82.95 & 91.84 / 90.31 / 90.31 \\
%      0.05 & 80.10 / 76.68 / 83.67 & 58.16 / 61.21 / 57.14 & 95.92 / 94.90 / 95.41\\
%      0.1 & 76.53 - 66.33 - 67.86 & 50 - 47.96 - 55.10 & 91.33 - 95.92 - 92.56 \\
%      0.5 & 53.06 / 44.33 / 42.35 & 44.39 / 44.39 / 59.18 & 92.35 / 91.33 / 93.37 \\
%      1 & 44.34 - 39.29 & 54.08 - 25 & 93.77 - 92.72 \\
%      \bottomrule
%    \end{tabular}
%  }
%  \caption{Test accuracy for FER classification and users- re-identification on CK+ subdatast with Different Noise Levels}
%  \label{tab:performance_metrics}
%\end{table}


\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.45\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/mobilenet_topk.pdf}
        \caption{Top-k results for user re-identification based on features extracted from the 4th Residual Block of \texttt{MobileNet} for the CK+ test subdataset}
        \label{fig:topkmobilnet}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/resnet_topk.pdf}
        \caption{Top-k results for user re-identification based on features extracted from the 4th Residual Block of \texttt{ResNet-9} for the CK+ test subdataset}
        \label{fig:topkresnet}
    \end{subfigure}
    \caption{Top-k Results for User Re-identification}
    \label{fig:topk-k}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{images/knn_real_faces.pdf}
  \caption{Examples of the ID-KNN prediction on the real-faces dataset.}
  \label{fig:knn_real}
\end{figure}


\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{images/knn_gen_faces.pdf}
  \caption{Examples of the ID-KNN prediction on the gen-faces dataset.}
  \label{fig:knn_gen}
\end{figure}

